The Optical Signatures of Stochastic Processes in Many-Body Exciton Scattering

We review our recent quantum stochastic model for spectroscopic lineshapes in the presence of a co-evolving and non-stationary background population of excitations. Starting from a field theory description for interacting bosonic excitons, we derive a reduced model whereby optical excitons are coupled to an incoherent background via scattering as mediated by their screened Coulomb coupling. The Heisenberg equations of motion for the optical excitons are then driven by an auxiliary stochastic population variable, which we take to be the solution of an Ornstein-Uhlenbeck process. Here we discuss an overview of the theoretical techniques we have developed as applied to predicting coherent non-linear spectroscopic signals. We show how direct (Coulomb) and exchange coupling to the bath give rise to distinct spectral signatures and discuss mathematical limits on inverting spectral signatures to extract the background density of states.

==> Headers.tex <==
\usepackage[numbers]{natbib}
\usepackage{url}
\setcounter{secnumdepth}{4}

% Metadata Information
\jname{Xxxx. Xxx. Xxx. Xxx.}
\jvol{AA}
\jyear{YYYY}
\doi{10.1146/((please add article doi))}


\usepackage{graphicx}% Include figure files
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage[utf8]{inputenc}
\usepackage{subfigure}
\usepackage{hyperref}
\usepackage{bbold}
\usepackage{bm}% bold math



\usepackage{mathptmx}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
%\usepackage{physics}





%\usepackage[normalem]{ulem} %to strike the words


\usepackage[T1]{fontenc}
\usepackage{mathptmx}
%\usepackage{xcolor}


%---TIKZ stuff

\usepackage{tikz}
\usetikzlibrary{positioning,calc}
\usetikzlibrary{trees}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{arrows.meta,decorations.pathreplacing}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

\tikzset{fontscale/.style = {font=\relsize{#1}}    }





\usepackage{color}
\definecolor{mma1}{rgb}{0.3725,0.5098,0.7020}
\definecolor{mma2}{rgb}{0.8745,0.6078,0.2039}
\definecolor{mma3}{rgb}{0.507813,0.714844,0.2039}
\definecolor{mma4}{rgb}{0.9137,0.3882,0.2398}
%-----EDITING COLORS-------
\definecolor{erb}{rgb}{0.3725,0.5098,0.7020}
\definecolor{hao}{rgb}{0.8745,0.6078,0.2039}
\definecolor{carlos}{rgb}{0.507813,0.714844,0.2039}
\definecolor{ajay}{rgb}{0.9137,0.3882,0.2398}
%-----EDITING COLORS--subs-------
% \definecolor{erb}{rgb}{0,0,0}
% \definecolor{hao}{rgb}{0,0,0}
% \definecolor{carlos}{rgb}{0,0,0}
% \definecolor{ajay}{rgb}{0,0,0}

% Include your paper's title here






